SpotFast Networks with Memory Augmented Lateral Transformers for Lipreading

This paper presents a novel deep learning architecture for word-level lipreading. Previous works suggest a potential for incorporating a pretrained deep 3D Convolutional Neural Networks as a front-end feature extractor. We introduce a SpotFast networks, a variant of the state-of-the-art SlowFast networks for action recognition, which utilizes a temporal window as a spot pathway and all frames as a fast pathway. We further incorporate memory augmented lateral transformers to learn sequential features for classification. We evaluate the proposed model on the LRW dataset. The experiments show that our proposed model outperforms various state-of-the-art models and incorporating the memory augmented lateral transformers makes a 3.7% improvement to the SpotFast networks.

==> dataset.tex <==
\section{Dataset}
We create a one-shot learning task for lipreading by repartitioning the Lip Reading in the Wild (LRW) dataset \cite{chung2016lip}. The original LRW dataset contains 500 words as a vocabulary set along with 488,766 training, 25,000 validation and 25,000 testing lip movements in the form of video clips. There are 29 video frames for every clip sequence.

We follow \cite{koch2015siamese} and partition the vocabulary set into 300 training, 100 validation and 100 testing. 

